Mechanistically analyzing the effects of fine-tuning on procedurally defined tasks

Fine-tuning large pre-trained models has become the de facto strategy for developing both task-specific and general-purpose machine learning systems, including developing models that are safe to deploy. Despite its clear importance, there has been minimal work that explains how fine-tuning alters the underlying capabilities learned by a model during pretraining: does fine-tuning yield entirely novel capabilities or does it just modulate existing ones? We address this question empirically in synthetic, controlled settings where we can use mechanistic interpretability tools (e.g., network pruning and probing) to understand how the model's underlying capabilities are changing. We perform an extensive analysis of the effects of fine-tuning in these settings, and show that: (i) fine-tuning rarely alters the underlying model capabilities; (ii) a minimal transformation, which we call a 'wrapper', is typically learned on top of the underlying model capabilities, creating the illusion that they have been modified; and (iii) further fine-tuning on a task where such hidden capabilities are relevant leads to sample-efficient 'revival' of the capability, i.e., the model begins reusing these capability after only a few gradient steps. This indicates that practitioners can unintentionally remove a model's safety wrapper merely by fine-tuning it on a, e.g., superficially unrelated, downstream task. We additionally perform analysis on language models trained on the TinyStories dataset to support our claims in a more realistic setup.

==> algorithms/algorithm_probe.tex <==
\begin{algorithm}[tb]
   \caption{Diversify-Aggregate-Repeat Training, DART}
   \label{alg:WATIG}
   
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} $M$ networks $f_{\theta^{k}}$ where $0<k \leq M$, whose weights are aggregated every $\lambda$ epochs. Training Dataset for each network $f_{\theta^{k}}$ is represented by ${D^{k}} =\{(x^{k}_i,y^{k}_i) \}$. The union of all datasets is denoted as ${D^{*}}$. Number of training epochs E, Maximum Learning Rate $\mathrm{LR}_{max}$, Cross-entropy loss $\ell_{CE}$. Model is trained using ERM for $E^{'}$ epochs initially.
   

\FOR{$epoch=1$ {\bfseries to} $E$}
    \STATE $\mathrm{LR} = 0.5  \cdot \mathrm{LR}_{max} \cdot (1 + cos((epoch -1)/E\cdot \pi))$
    \IF{ $epoch<E'$}
    \STATE $\theta = min_{\theta}\frac{1}{n}\sum\limits_{i=1}^n\ell_{CE}(\theta,{D^{*}})$ 
        \ELSE
        \IF{$epoch=E'$}
   \STATE $\theta^{k}\leftarrow \theta ~~ \forall k\in [1,M]$ 
        \ENDIF
      \STATE  $\theta^{k} = min_{\theta^{k}}\frac{1}{n}\sum\limits_{i=1}^n\ell_{CE}(\theta,{D^{k}})$ $\forall k \in [1,M]$ 
    
\IF{ $epoch ~ \%~\lambda=0$}
    \STATE $\theta = \frac{1}{M}\sum\limits_{k=1}^M\theta^{k}$ 
   \STATE $\theta^{k}\leftarrow \theta ~~ \forall k\in [1,M]$ 
\ENDIF
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> algorithms/algorithm_prune.tex <==
\begin{algorithm}[tb]
   \caption{Pruning protocol utlized}
   \label{alg:WATIG}
   
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} $M$ networks $f_{\theta^{k}}$ where $0<k \leq M$, whose weights are aggregated every $\lambda$ epochs. Training Dataset for each network $f_{\theta^{k}}$ is represented by ${D^{k}} =\{(x^{k}_i,y^{k}_i) \}$. The union of all datasets is denoted as ${D^{*}}$. Number of training epochs E, Maximum Learning Rate $\mathrm{LR}_{max}$, Cross-entropy loss $\ell_{CE}$. Model is trained using ERM for $E^{'}$ epochs initially.
   

\FOR{$epoch=1$ {\bfseries to} $E$}
    \STATE $\mathrm{LR} = 0.5  \cdot \mathrm{LR}_{max} \cdot (1 + cos((epoch -1)/E\cdot \pi))$
    \IF{ $epoch<E'$}
    \STATE $\theta = min_{\theta}\frac{1}{n}\sum\limits_{i=1}^n\ell_{CE}(\theta,{D^{*}})$ 
        \ELSE
        \IF{$epoch=E'$}
   \STATE $\theta^{k}\leftarrow \theta ~~ \forall k\in [1,M]$ 
        \ENDIF
      \STATE  $\theta^{k} = min_{\theta^{k}}\frac{1}{n}\sum\limits_{i=1}^n\ell_{CE}(\theta,{D^{k}})$ $\forall k \in [1,M]$ 
    
\IF{ $epoch ~ \%~\lambda=0$}
    \STATE $\theta = \frac{1}{M}\sum\limits_{k=1}^M\theta^{k}$ 
   \STATE $\theta^{k}\leftarrow \theta ~~ \forall k\in [1,M]$ 
\ENDIF
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> tables/table_summary.tex <==
\begin{table*}[h]
\caption{\textbf{Reference table for all results in appendix.} For ease of reference, we summarize the experiment titles, takeaways, and figure/table identifiers for all results in the appendix.}
\setlength\tabcolsep{2pt}
\centering
\resizebox{1.0\linewidth}{!}{
\centering
\label{table:table_summary}
\begin{tabular}{l|l|l|l}
\toprule
Setup & Experiment                                                                                    & \multicolumn{1}{l|}{Takeaway}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & Figures / Table Refs  \\ 
\hline
  & \begin{tabular}[l]{@{}l@{}} Impact of pretraining sampling  \\ prior on fine-tuning task accuracy            \end{tabular}                  &  \begin{tabular}[l]{@{}l@{}} Presence of the strongly relevant capability inhibits the learning of spurious \\ correlations and absence of strongly relevant capability enhances the learning \\ of spurious correlations. On using small learning rate $\eta_{S}$, in the \\ absence of strongly relevant capability, the model is not able to learn a new \\ capability but can still learn spurious correlations.    \end{tabular}                                                                                                                                                                                                                                                                                                                                                                     & Fig.~\ref{fig:pcfg_count_supp_effect_lr_200k}, \ref{fig:pcfg_index_supp_effect_lr_200k}, \ref{fig:pcfg_count_supp_ws_200k}, \ref{fig:pcfg_index_supp_ws_200k}, \ref{fig:pcfg_count_supp_ws_50k}, \ref{fig:pcfg_index_supp_ws_50k},\ref{fig:pcfg_count_supp_ws_10k}, \ref{fig:pcfg_index_supp_ws_10k}, \ref{fig:pcfg_mix_data_0p999_pt}, \ref{fig:pcfg_mix_data_0p999_ft}, \ref{fig:pcfg_mix_data_0p5_pt}, \ref{fig:pcfg_mix_data_0p5_ft}         \\ \cline{2-4}

    & \begin{tabular}[l]{@{}l@{}} Jailbreaking Analysis    \end{tabular}                  &  \begin{tabular}[l]{@{}l@{}} We can jailbreak the fine-tuning filter thus showing that old capabilities \\are not lost on fine-tuning  \end{tabular}                                                                                                                                                                                                                                                                                                                                                                     & Fig.~\ref{fig:pcfg_jailbreak}  \\ \cline{2-4}
      & \begin{tabular}[l]{@{}l@{}} Impact of pretraining sampling \\ prior on pretraining task accuracy   \end{tabular}                           & \begin{tabular}[l]{@{}l@{}} The drop in pre-training task performance is maximum if fine-tuning capabilities \\ are not already present in the model. This drop is further enhanced in presence \\ of spurious correlations. \end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           & Fig.~\ref{fig:pcfg_count_supp_rc_count_ws0}, \ref{fig:pcfg_index_supp_rc_count_ws0}, \ref{fig:pcfg_count_supp_rc_count_ws1}, \ref{fig:pcfg_index_supp_rc_count_ws1}, \ref{fig:pcfg_count_supp_rc_count_ws0_small}, \ref{fig:pcfg_index_supp_rc_count_ws0_small}, \ref{fig:pcfg_count_supp_rc_count_ws1_small}, \ref{fig:pcfg_index_supp_rc_count_ws1_small}                   \\ \cline{2-4}
      PCFG ~~ & Capability revival on reverse fine-tuning                                                     & \begin{tabular}[l]{@{}l@{}}In presence of a strongly relevant fine-training capability, the model quickly \\ regains its pretraining capability on reverse fine-tuning.  In the absence of strongly \\ relevant capability revival is less sample efficient but still fairly fast.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & Fig.~\ref{fig:pcfg_count_supp_cr_200k}, \ref{fig:pcfg_count_supp_cr_50k}, \ref{fig:pcfg_count_supp_cr2_200k}    , \ref{fig:pcfg_reft_adv}, \ref{fig:pcfg_reft_all}          \\ \cline{2-4}
      & \begin{tabular}[l]{@{}l@{}}  Pruning the model trained using low value of \\fine-tuning sampling prior during pre-training \end{tabular}               & \begin{tabular}[l]{@{}l@{}}Pruning off the neurons learning the wrapper to minimally alter the weakly \\ relevant pretraining capability  leads to the revival of the pre-training capability.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & Fig.~\ref{fig:pcfg_count_supp_prune_neuron}, \ref{fig:pcfg_index_supp_prune_neuron}, \ref{fig:pcfg_index_supp_prune_index_new}, \ref{fig:pcfg_count_supp_prune_prob}, \ref{fig:pcfg_index_supp_prune_prob}, \ref{fig:pcfg_count_supp_prune_prob_neuron}, \ref{fig:pcfg_index_supp_prune_prob_neuron}                  \\ \cline{2-4}
      & \begin{tabular}[l]{@{}l@{}} Pruning the model trained using high value of \\  fine-tuning sampling prior during pre-training         \end{tabular}        & \begin{tabular}[l]{@{}l@{}}Pruning off the neurons learning an inhibitor to suppress the strongly relevant \\ pretraining capability which was not  used during fine-tuning leads to the revival \\ of the pre-training capability.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           & Fig.~\ref{fig:pcfg_count_supp_inhibitor}, \ref{fig:pcfg_index_supp_inhibitor}, \ref{fig:pcfg_count_supp_inhibitor2}, \ref{fig:pcfg_index_supp_inhibitor2}                 \\ \cline{2-4}
      & Probing analysis on fine-tuned model                                                          & \begin{tabular}[l]{@{}l@{}}Using a small learning rate $\eta_{S}$ in the absence of strongly relevant fine-tuning capability \\ leads-wEP231F to the retention of the pretraining capabilities. If fine-tuning is carried out \\ in the presence of spurious correlations, the pre-training capabilities are retained \\ for large learning rate also. \end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              &  
      Fig.~\ref{fig:pcfg_count_supp_prob}, \ref{fig:pcfg_index_supp_prob}, \ref{fig:pcfg_count_supp_prob_50k}, \ref{fig:pcfg_count_supp_prob_200k_a}, \ref{fig:pcfg_count_supp_prob_200k_b}, \ref{fig:pcfg_index_supp_prob_50k}, \ref{fig:pcfg_index_supp_prob_200k_a}, \ref{fig:pcfg_index_supp_prob_200k_b}, T\ref{fig:pcfg_mix_data_0p999_probe}, \ref{fig:pcfg_mix_data_0p5_probe}, \ref{fig:pcfg_jailbreak_probe}
      \\
      \hline
 & \begin{tabular}[l]{@{}l@{}}  Are new capabilities learned on fine-tuning? \\  - attention map visualization \end{tabular} & \begin{tabular}[l]{@{}l@{}}In counting task, the model can learn new capability on using $\eta_{M}$, $\eta_{L}$, but not \\ on using $\eta_{S}$.  On using $\eta_{S}$ and in presence  of spurious correlations  model learns\\  a wrapper on its compiled capability. In case of max-element task, since \\ the mechanism required to perform well on fine-tuning task is already \\  present in the compiled model, using $\eta_{S}$ leads to learning of the fine\\tuning task. This happens even in the presence of spurious correlations. \end{tabular} & Fig.~ \ref{fig:tracr_count_supp_untuned}, 
 
 \ref{fig:tracr_high_lr},\ref{fig:tracr_count_supp_val_three_eg}, \ref{fig:tracr_plot_max_element}, \ref{fig:tracr_count_supp_all_count}, \ref{fig:tracr_max_supp_all_three}, \ref{fig:tracr_max_supp_diff2}, \ref{fig:tracr_max_supp_all}, 
Table~\ref{table:tracr_count}      \\ \cline{2-4} Tracr ~~~
      & \begin{tabular}[l]{@{}l@{}} Are old capabilities lost on fine-tuning? \\ - attention map visualization \end{tabular}  & \begin{tabular}[l]{@{}l@{}} Capability revival is possible even on using small and very small learning rate \\ for reverse fine-tuning thus indicating that the pre-trained capabilities are not \\ lost on fine-tuning using medium or lower learning rate.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           & Fig.~\ref{fig:tracr_count_supp_revival}, \ref{fig:tracr_cr},  \ref{fig:tracr_count_supp_act_tuned}, \ref{fig:tracr_count_supp_act}, \ref{fig:tracr_count_cap_rev_all_three}, \ref{fig:tracr_count_supp_diff_rtrain}, \ref{fig:tracr_count_cap_rev_all_three}, \ref{fig:pcfg_reft_tracr} Table~\ref{table:tracr_count_reft}                \\ \cline{2-4}
      & Pruning analysis  & \begin{tabular}[l]{@{}l@{}} Pruning off a single weight leads to the revival of compiled capability, thus \\ demonstrating that a single weight can learn a wrapper on model's \\ compiled capabilities. \end{tabular} & Fig.~\ref{fig:tracr_prune_lrs}, \ref{fig:tracr_count_supp_prune_0p5_0p8}, \ref{fig:tracr_count_supp_prune_weight}, \ref{fig:tracr_count_supp_prune_neuron}, \ref{fig:tracr_count_supp_hist}
\\
  \hline
  
   
      & \begin{tabular}[l]{@{}l@{}} Impact of fine-tuning on pre-training task  \\ performance \end{tabular}  & \begin{tabular}[l]{@{}l@{}} Using larger learning rate leads to a more pronounced increase in loss and \\ loss of generative capability on pre-training task.  \end{tabular} & Fig.~ \ref{fig:tinystorieslossdeletion}, \ref{fig:tinystoriesgptdeletion}             \\ \cline{2-4} Tiny Stories ~~~
      & \begin{tabular}[l]{@{}l@{}} Capability revival analysis on reverse fine-tuning \end{tabular}  & \begin{tabular}[l]{@{}l@{}} Reverse fine-tuning easily recovers the pre-training capability to generate stories \\ with the desired features. \end{tabular} & Fig.~\ref{fig:tinystorieslossrecovery} , \ref{fig:tinystoriesgptrecovery}   \\ \cline{2-4}
      & Probing analysis  & \begin{tabular}[l]{@{}l@{}} For different features present in tiny stories, the probing analysis shows that \\ regardless of the deletion protocol used model's capability to generate \\ features learned during pre-training is not lost. \end{tabular} & Fig. \ref{fig:tinystoriesprobe2}, \ref{fig:tinystoriesprobefeat1}, \ref{fig:tinystoriesprobefeat2}, \ref{fig:tinystoriesprobefeat3}   
\\
\bottomrule
\end{tabular}
}

\end{table*}






==> tables/tiny_stories_nowrap.tex <==
 % \begin{table}[]
 % \centering
 % \caption{\textbf{TinyStories Reverse Fine-tuning Analysis}. Loss on generating twists, after deletion and then recovery of the twist capability. In deletion types, F, AT and S stand for Filtering (fine-tunes the model on a dataset where all instances of stories with twists are filtered out), Adversarial Training (adds the ``Twist'' instruction to the prompt for stories that do not contain twists) and Specialisation (filters the dataset to only include stories containing another, unrelated feature). Only with a large learning rate does loss jump significantly after deletion, and for this learning rate recovery of the capability is not as strong as learning the capability from scratch from a pretrained model.
 % }
 % \label{tab:tinystoriesresults}
 % \begin{tabular}{@{}rlll|lll@{}}
 % \toprule
 % \multicolumn{1}{l}{}                   & \multicolumn{1}{l}{Loss} & \multicolumn{1}{l}{After}  & \multicolumn{1}{l|}{Deletion}  & \multicolumn{1}{l}{Loss} & \multicolumn{1}{l}{After} & \multicolumn{1}{l}{Recovery} \\ \midrule
 % \multicolumn{1}{l}{}                   & \multicolumn{1}{l}{LR}       & \multicolumn{1}{l}{}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 % Deletion Type                              & 0.00001                      & 0.0001                & 0.001                  & 0.00001                      & 0.0001               & 0.001                \\ \midrule
 % F                                      & 0.79                     & 0.82              & 0.99               & 0.71                     & 0.71             & 0.78             \\
 % F + AT                                 & 0.79                     & 0.83              & 1.01                & 0.71                     & 0.71             & 0.78             \\
 % F + S                                  & 0.81                     & 0.86              & 1.02               & 0.71                     & 0.72             & 0.79             \\
 % F + S + AT                             & 0.81                     & 0.86              & 1.07               & 0.71                     & 0.72             & 0.79             \\ \midrule
 % \multicolumn{1}{l}{Not in Pretraining} & \multicolumn{1}{l}{-}        & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & 0.75                     & 0.75             & 0.75             \\ \bottomrule
 % \end{tabular}
 % \end{table}


\setlength\intextsep{1pt}
\begin{table}
\small
\centering
\begin{tabular}{@{}r|llll@{}}
\toprule
Deletion Type                   & \multicolumn{4}{c}{Twist Proportion at Iteration}  \\ \midrule
  & 0 & 30 & 300 & 3000 \\ \midrule
$\mathtt{F}$ ($\eta_M$) & 44\% & 81\% & 81\% & 82\% \\
$\mathtt{F+R}$ ($\eta_M$) & 12\% & 56\% & 69\% & 75\% \\
$\mathtt{F+MM}$ ($\eta_M$) & 31\% & 88\% & 50\% & 75\% \\ \midrule
$\mathtt{F}$ ($\eta_S$) & 69\% & 88\% & 75\% & 94\% \\
$\mathtt{F+R}$ ($\eta_S$) & 12\% & 44\% & 81\% & 81\% \\
$\mathtt{F+MM}$ ($\eta_S$) & 50\% & 81\% & 62\% & 81\% \\ \midrule
Not in $\mathtt{PT}$ & 12\% & 31\% & 44\% & 81\% \\ \bottomrule
\end{tabular}
\vspace{0.1cm}
\caption{\textbf{TinyStories \reft{} Analysis}. We report the percent of generations with a $\mathtt{twist}$ during reverse fine-tuning for the twist capability. $\mathtt{F}$, $\mathtt{R}$, and $\mathtt{MM}$ stand for our three fine-tuning protocols: Filtering, Randomisation and Mix \& Match (see App.~\ref{appendix:tinystories} for details). Regardless of learning rate and protocol, models relearn to generate stories with $\mathtt{twist}$ more sample-efficiently than the control model pre-trained on data w/o twists and fine-tuned to generate them (Not in $\mathtt{PT}$).}
% \vspace{-2pt}
\label{tab:tinystoriesresults}
\end{table}

==> tables/tracr_count_max.tex <==
\begin{table*}[t]
\caption{\textbf{Results on counting and max element task tracr setups.} The evaluation is done on test sets with and without the spurious correlation and the tracr compiled models are fine-tuned for different learning rates and  different value of $C_{Tr}$.}
\label{table:tracr_count}
\caption{\textbf{Tracr Results}}
\setlength\tabcolsep{1pt}
\resizebox{1.0\linewidth}{!}{
\label{table:tracr_max_element}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{3}{*}{$\eta$}       & \multirow{3}{*}{$R_{train}$}  & \multicolumn{4}{|c}{Counting Element}         &        \multicolumn{4}{|c}{Max Identifier}                   \\
\cline{3-10}
         &          & \multicolumn{2}{|c|}{$R_{test}=1$}                   & \multicolumn{2}{|c}{$R_{test}=0$}              & \multicolumn{2}{|c|}{$R_{test}=1$}                   & \multicolumn{2}{|c}{$R_{test}=0$}              \\
        \cline{3-10}
         &          & Acc$_{pt}$      & Acc$_{ft}$  & Acc$_{pt}$  & Acc$_{ft}$  & Acc$_{pt}$       & Acc$_{ft}$  & Acc$_{pt}$  & Acc$_{ft}$  \\
         \midrule
1e-1 & 0        & 0.0  & 100.0 & 0.0  & 100.0 & 20.3 & 34.5 & 0.0  & 99.3 \\
         & 1        & 0.0  & 100.0 & 35.8 & 0.7   & 0.3  & 99.6 & 16.8 & 37.8 \\
1e-2 & 0        & 1.1  & 96.3  & 0.0  & 98.8  & 29.7 & 0.2  & 16.3 & 52.6 \\
         & 1        & 0.3  & 98.3  & 4.2  & 0.2   & 11.1 & 78.5 & 23.8 & 14.4 \\
1e-3 & 0        & 54.6 & 1.2   & 25.7 & 27.2  & 6.4  & 20.2 & 4.5  & 28.5 \\
         & 1        & 4.0  & 94.3  & 10.3 & 2.2   & 16.0 & 33.2 & 12.8 & 14.0 \\
1e-4 & 0        & 32.6 & 0.0   & 10.6 & 28.7  & 0.5  & 82.6 & 0.5  & 91.1 \\
         & 1        & 1.6  & 98.3  & 10.6 & 0.2   & 0.0  & 90.2 & 0.7  & 88.6   \\
\bottomrule
\end{tabular}
}
\end{table*}[t]

% \end{wraptable}






% \setlength\intextsep{1pt}
% \begin{wraptable}{R}{6.8cm}
% \centering
% \footnotesize
%     \vspace{-0em}
%     \begin{tabular}{@{}l@{\hskip 6pt} c cc@{}}
%     \toprule
%       \,  & Hessian & Dim.\ & Complete\\
%       \midrule
%         \, InfoNCE
%         & $A_0$ & 4 & 4 \\
%         \, NT-Xent (SimCLR)
%         & $A_0 - \nicefrac{C}{N}$ & 4 & 4 \\
%         \, Spectral Contrastive
%         & $C$ & 4 & 4 \\
%         \, Barlow Twins
%         & $A_0 + C$ & 4 & 4 \\
%         \, + Normalization
%         & - & 4 & 4\\
%         \, \quad + bias
%         & - & 4 & 4\\
%         \, + Weight Decay
%         & $+ \gamma I$ & 4 & 4\\
%     \bottomrule
%     \end{tabular}
% \vspace{-0.5em}
%     \caption{\small \textbf{What shapes the SSL landscapes around the origin?} 
%     For each of the SSL losses, the combination of data covariance ($A_0$), data-augmentation covariance ($C$), and dataset size ($N$) can affect its stability and thus determine the presence (4) and absence (4) of dimensional/complete collapse (Here, a 4 means ``there exists a hyperparameter setting and data distribution such that the relevant collapse happens;'' see \autoref{sec: theory}). Beyond collapses, the theory implies that SCL, whose landscape is formed primarily by data augmentation, is more robust to data imbalance than InfoNCE, which is affected primarily by the data (see \autoref{sec: implications}).
%     }
%     \vspace{-1.5em}
%     \label{tab:sumary}
% \end{wraptable}
